Teechain: A Secure Payment Network with Asynchronous Blockchain Access

Blockchains such as Bitcoin and Ethereum execute payment transactions securely, but their performance is limited by the need for global consensus. Payment networks overcome this limitation through off-chain transactions. Instead of writing to the blockchain for each transaction, they only settle the final payment balances with the underlying blockchain. When executing off-chain transactions in current payment networks, parties must access the blockchain within bounded time to detect misbehaving parties that deviate from the protocol. This opens a window for attacks in which a malicious party can steal funds by deliberately delaying other parties' blockchain access and prevents parties from using payment networks when disconnected from the blockchain. We present Teechain, the first layer-two payment network that executes off-chain transactions asynchronously with respect to the underlying blockchain. To prevent parties from misbehaving, Teechain uses treasuries, protected by hardware trusted execution environments (TEEs), to establish off-chain payment channels between parties. Treasuries maintain collateral funds and can exchange transactions efficiently and securely, without interacting with the underlying blockchain. To mitigate against treasury failures and to avoid having to trust all TEEs, Teechain replicates the state of treasuries using committee chains, a new variant of chain replication with threshold secret sharing. Teechain achieves at least a 33x higher transaction throughput than the state-of-the-art Lightning payment network. A 30-machine Teechain deployment can handle over 1 million Bitcoin transactions per second.

==> algo2.tex <==
% Algorithm:
%\newpage
%\onecolumn
\begin{algorithm*}[t]\scriptsize
	\caption{\sys multi-hop payment protocol execution at TEE $p_i$ {\footnotesize (For brevity, we omit encryption, integrity and freshness
            protection of messages. TEEs in the path are numbered
            $1\ldots{}n$. Overlined variables are signed by the corresponding private key. $\bot$ represents null.)}} 
	\label{alg:teechainA}
	\SetAlgoNoEnd
	\DontPrintSemicolon 
	\SetNoFillComment
	\SetKw{assert}{assert}
	\SetInd{0.4em}{0.4em}
%	\vspace*{-2em}
	\begin{multicols}{4}
	%\commentx{} \;\BlankLine 
	% $\nodePubKeys \gets ()$ \; 
 	\assign{\signedChainSettleTx_{i}}{\bot}\; 
 	\assign{amnt_{i}}{\bot}\;\BlankLine 
	
	\KwOn({\cmdRoutePayment($\mathit{amount}, \fromto{p_1}{p_n}$)}) {\label{alg:routepayment} 
 		% \; \label{alg:route:stage}\label{alg:route:balance}
 		\send{p_1}{\cmdLockAlg, amount, \fromto{p_1}{p_n}, \chainSettleTx()}
% 		assert $\stage(id(\langle p_1, p_2\rangle)) = \stageIdle$ \; 
% 		assert { $\channelMyBalance(id(\langle p_1, p_2\rangle)) \geq \textit{amount}$} \;\label{alg:route:balance}
		%   $\nodePubKeys \gets (p_1, \dots, p_n)$ \;
% 		send $(\cmdLockAlg, (p_1, \dots, p_n), \chainSettleTx())$ encrypted and signed for $p_2$ 
	}\BlankLine 
	
	\KwOn({\cmdReceive($\cmdLockAlg, \mathit{amount},\linebreak \fromto{p_1}{p_n}, \chainSettleTx(\fromto{p_1}{p_{i-1}})$)}) {\label{alg:receive:lock}
% 		assert $\stage(id(\langle p_{i}, p_{i+1}\rangle)) = \stageIdle$ \;
		%   $\nodePubKeys \gets (p_1, \dots, p_n)$ \;		
 		\assertx{
 			\channel{stage}{p_i}{p_{i+1}} = \stageIdle
 		}\;
 		\assertx{
  			\channel{myBal}{p_i}{p_{i+1}} \geq amount
 		}\;
 		\assign{amnt_{i}}{amount} \;
 		
		\If{$i < n$} {
% 			$\stage(id(\langle p_{i}, p_{i+1}\rangle)) \gets \stageLocked$ \;
% 			send $(\cmdLockAlg, (p_1, \dots, p_n), \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{i-1}, p_{i}\rangle))$ encrypted and signed for $p_{i + 1}$ \label{alg:settletx}
			\assign{\channel{stage}{p_i}{p_{i+1}}}{\cmdLockAlg} \;
			\sendhack{p_{i+1}}\linebreak{\cmdLockAlg, \fromto{p_1}{p_n},\chainSettleTx(\fromto{p_1}{p_{i}})})
			\label{alg:lock:send}
		} \Else({ \commentx{$i == n$ }}) {
% 			$\stage(id(\langle p_{n-1}, p_{n}\rangle)) \gets \stageSigned$ \; \label{alg:sign:start}
% 			send $(\cmdSign, \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{n-1}, \underline{p_{n}}\rangle))$ encrypted and signed for $p_{n - 1}$
			\assign{\channel{stage}{p_{n-1}}{p_n}}{\cmdSignAlg}\; \label{alg:sign:start}
			\send{p_{n-1}}{\cmdSignAlg, \chainSettleTx(\fromto{p_1}{p_{n-1}}, \signed{p_{n}})}
			\label{alg:sign:send}
		}
		
	}
	
	% \KwOn({Command \textit{cmd} at stage \stageIdle}) {
	%     \If({\hfill (First in chain)})
	%             {$\textit{cmd} = (\cmdLockAlgNewChain, (p_1, p_2, \dots, p_n))$ and $i = 1$}{ 
	%         $\stage \gets \stageLocked$ \; 
	%         $\nodePubKeys \gets (p_1, \dots, p_n)$ \; 
	%         return $(\cmdLockAlg, (p_1, \dots, p_n), \chainSettleTx())$ encrypted and signed for $p_2$. 
	%     } 
	% 
	%     \If{$\textit{cmd} = (\cmdLockAlg, (p_1, \dots, p_n), \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{i-2}, p_{i-1}\rangle))$, encrypted and signed by $p_{i-1}$}{ 
	%         $\nodePubKeys \gets (p_1, \dots, p_n)$ \; 
	%         \If{$i < n$} {
	%             $\stage \gets \stageLocked$ \; 
	%             return $(\cmdLockAlg, (p_1, \dots, p_n), \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{i-1}, p_{i}\rangle))$ encrypted and signed for $p_{i + 1}$. 
	%         } \Else({($i = n$)}) {
	%             $\stage \gets \stageSigned$ \; 
	%             return $(\cmdSignAlg, \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{n-1}, \underline{p_{n}}\rangle))$ encrypted and signed for $p_{n - 1}$. 
	%         }
	%     } 
	% }
	% %\BlankLine
	\vfill\null
	\KwOn({\cmdReceive($\cmdSignAlg, 
		\chainSettleTx(\fromto{p_1}{p_{i}}, \fromto{\signed{p_{i+1}}}{\signed{p_{n}}})$)}) {\label{alg:sign}
		\assertx{
			\channel{stage}{p_i}{p_{i+1}} = \cmdLockAlg
		} \;
		\If{$i > 1$} { 
			\assign{\channel{stage}{p_i}{p_{i+1}}}{\cmdSignAlg} \; 
			\sendhack{p_{i-1}}\linebreak{\cmdSignAlg, \chainSettleTx(\fromto{p_1}{p_{i-1}}, \fromto{\signed{p_{i}}}{\signed{p_{n}}})}) \; \label{alg:sign:send2}
		} \Else({ \commentx{ $i == 1$ } }) { 
			\assign{\signedChainSettleTx_{1}}{\chainSettleTx(\fromto{\signed{p_1}}{\signed{p_{n}}})} \; \label{alg:signed:done}			
			\assign{\channel{stage}{p_1}{p_2}}{\cmdPromiseAAlg} \; \label{alg:promiseA:start}
			\send{p_2}{\cmdPromiseAAlg, \signedChainSettleTx_{1})} \; \label{alg:promiseA:sendfirst}
		}
	}\BlankLine 
	
	
	% \KwOn({Command \textit{cmd} at stage \stageLocked}) {
	%     $\textit{cmd} = (\cmdSign, \chainSettleTx(p_1, \dots, p_i, \underline{p_{i+1}}, \dots, \underline{p_n}))$, encrypted and signed by $p_{i+1}$ \;
	%     \If{$\textit{cmd} = (\cmdSign, 
	%             \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{i-1}, p_{i}\rangle, \langle p_{i}, \underline{p_{i+1}}\rangle, \dots, \langle \underline{p_{n-1}}, \underline{p_{n}}\rangle))$, encrypted and signed by $p_{i+1}$}{ 
	%         \If{$i > 1$} { 
	%             $\stage \gets \stageSigned$ \; 
	%             return $(\cmdSign, \chainSettleTx(\langle p_1, p_2\rangle, \dots, \langle p_{i-1}, \underline{p_{i}}\rangle, \langle \underline{p_{i}}, \underline{p_{i+1}}\rangle, \dots, \langle \underline{p_{n-1}}, \underline{p_{n}}\rangle))$ encrypted and signed for $p_{i - 1}$ \; 
	%         } \Else({($i = 1$)}) { 
	%             $\signedChainSettleTx \gets \chainSettleTx(\langle \underline{p_1}, \underline{p_2}\rangle, \dots, \langle \underline{p_{n-1}}, \underline{p_{n}}\rangle))$ \; 
	%             $\stage \gets \stagePromisedA$ \; 
	%             return $(\cmdPromiseA, \signedChainSettleTx)$ encrypted and signed for $p_{i+1}$ \; 
	%         } 
	%     } 
	%     
	%     \If{$\textit{cmd} = \cmdEject$} {
	%         $\stage \gets \stageTerminated$ \; 
	%         return pre-payment settlements for channels with $p_{i-1}$ and $p_{i+1}$ (or just one if at end of chain) \;
	%     }
	% } 
	% %\BlankLine
	
	\KwOn({\cmdReceive$(\cmdPromiseAAlg, \signedChainSettleTx)$}) { \label{alg:receive:promiseA}
	
		\assertx {
			\channel{stage}{p_i}{p_{i+1}} = \cmdSignAlg
		} \;
		
		\assign{\signedChainSettleTx_{i}}{\signedChainSettleTx} \label{alg:sign:done2}\; 
		
		\If{$i < n$} { 
			\assign{\channel{stage}{p_i}{p_{i+1}}}{\cmdPromiseAAlg} \label{alg:promiseA:start2}\; 
			\send{p_{i+1}}{\cmdPromiseAAlg, \signedChainSettleTx}. \label{alg:promiseA:send}
		} \Else({ \commentx{ $i == n$ } }) {
			\assign{\channel{stage}{p_{n-1}}{p_n}}{\cmdPromiseBAlg} \; \label{alg:promiseB:start}
			\assign{\channel{myBal}{p_n}{p_{n-1}}}{\channel{myBal}{p_n}{p_{n-1}} + amnt_{i}} \; \label{alg:promiseB:update1}
			\send{p_{n-1}}{\cmdPromiseBAlg} \label{alg:promiseB:sendfirst} 
		} 
	}\BlankLine 
	
	
	% \KwOn({Command \textit{cmd} at stage \stageSigned}) { 
	%     \If{$\textit{cmd} = (\cmdPromiseA, \textit{signedTx})$ encrypted and signed by $p_{i-1}$}{ 
	%         $\signedChainSettleTx \gets \textit{signedTx}$ \; 
	%         \If{$i < n$} { 
	%             $\stage \gets \stagePromisedA$ \; 
	%             return $(\cmdPromiseA, \signedChainSettleTx)$ encrypted and signed for $p_{i+1}$. 
	%         } \Else({($i = n$)}) {
	%             $\stage \gets \stagePromisedB$ \; 
	%             return \cmdPromiseBAlg encrypted and signed for $p_{n - 1}$. 
	%         } 
	%     } 
	% 
	%     \If{$\textit{cmd} = \cmdEject$} {
	%         $\stage \gets \stageTerminated$ \; 
	%         return pre-payment settlements for channels with $p_{i-1}$ and $p_{i+1}$ (or just one if at end of chain) \;
	%     }
	% } 
% 	\rememberlines
	%\end{algorithm*}
	%
	%\begin{algorithm*}[t] 
	%	\caption{\sys Trusted Execution at node $p_i$ (2/2)} 
	%	\label{alg:teechainB} 
	%	\SetAlgoNoLine 
	%	\SetAlgoNoEnd 
	%	\DontPrintSemicolon 
	%	\SetNoFillComment
	%	\resumenumbering 
	
	\KwOn({\cmdReceive$(\cmdPromiseBAlg)$}) { \label{alg:receive:promiseB}
		
		\assertx {
			\channel{stage}{p_i}{p_{i+1}} = \cmdPromiseAAlg
		} \;
		
		\If{$i > 1$} { 
			\assign{\channel{stage}{p_i}{p_{i+1}}}{\cmdPromiseBAlg} \;
			\assign{\channel{myBal}{p_i}{p_{i+1}}}{\channel{myBal}{p_i}{p_{i+1}} + amnt_{i}} \label{alg:promiseB:update_one} \;
			\assign{\channel{myBal}{p_i}{p_{i-1}}}{\channel{myBal}{p_i}{p_{i-1}} - amnt_{i}} \label{alg:promiseB:update_two} \; 
			\send{p_{i-1}}{\cmdPromiseBAlg} \; \label{alg:promiseB:send}
		} \Else({ \commentx{ $i == 1$ }}) {
			\assign{\signedChainSettleTx_{1}}{\bot}   \; \label{alg:deletetransaction:start}
			\assign{\channel{stage}{p_1}{p_2}}{\cmdUpdateAlg} \;  \label{alg:update:start}
			\send{p_2}{\cmdUpdateAlg} \; 
		}
	}\;
	%\BlankLine
	
	\KwOn({\cmdReceive$(\cmdUpdateAlg)$}) {
		\label{alg:release}
		
		\assertx {
			\channel{stage}{p_i}{p_{i+1}} = \cmdPromiseBAlg \;
		}
		
		\If{$i < n$} {
			\assign{\signedChainSettleTx_{i}}{\bot}   \; \label{alg:update:discard}
			\assign{\channel{stage}{p_i}{p_{i+1}}}{\cmdUpdateAlg} \;
			\label{alg:update:post-payment}
			\send{p_{i+1}}{\cmdUpdateAlg} \label{alg:update:send}
		} \Else({ \commentx{ $i == n$ } }) {
			\assign{\channel{stage}{p_{n-1}}{p_n}}{\stageIdle} \; \label{alg:release:start}
			\send{p_{n-1}}{\cmdReleaseAlg} \; \label{alg:release:sendfirst} } 
	}\BlankLine 
	%\BlankLine
	
	
	% \KwOn({Command \textit{cmd} at stage \stagePromisedA}) { 
	%     \If{$\textit{cmd} = \cmdPromiseB$, encrypted and signed by $p_{i+1}$}{ 
	%         \If{$i > 1$} { 
	%             $\stage \gets \stagePromisedB$ \; 
	%             return \cmdPromiseB encrypted and signed for $p_{i - 1}$ \; 
	%         } \Else({($i = 1$)}) { 
	%             $\stage \gets \stageIdle$ \; 
	%             return \cmdReleaseAlg encrypted and signed for $p_{i+1}$ \; 
	%         } 
	%     } 
	%     
	%     \If{$\textit{cmd} = \cmdEject$} {
	%         return \signedChainSettleTx \;
	%         $\stage \gets \stageTerminating$ \;
	%     }
	% }
	% %\BlankLine
	
	\KwOn({\cmdReceive$(\cmdReleaseAlg)$}) { \label{alg:receive:release}
		
		\assertx {
			\channel{stage}{p_i}{p_{i+1}} = \cmdUpdateAlg
		} \;  \label{alg:deletetransaction:again}
		
		\assign{\channel{stage}{p_i}{p_{i+1}}}{\stageIdle} \; 
		
		\If{$i > 1$} {
			\send{p_{i-1}}{\cmdReleaseAlg} 
		} 
	}\BlankLine 
	%\BlankLine
	
	% \KwOn({Command \textit{cmd} at stage \stagePromisedB}) {
	%     \If{$\textit{cmd} = \cmdRelease$ encrypted and signed by $p_{i-1}$}{ 
	%         $\stage \gets \stageIdle$ \; 
	%         \If{$i < n$} {
	%             return $\cmdRelease$ encrypted and signed for $p_{i+1}$. 
	%         } 
	%     } 
	%     \If{\textit{cmd} = \cmdEject} { 
	%         return local post-payment settlements \; 
	%         $\stage \gets \stageTerminated$ \; 
	%     }
	% }
	% \BlankLine
	
	% \KwOn({Command \textit{cmd} at stage \stageTerminating}) {
	%     \If{$\textit{cmd} = (\cmdEject, \textup{pre-payment transaction of any channel in the chain})$} {
	%         $\stage \gets \stageTerminated$ \; 
	%         return pre-payment settlements for channels with $p_{i-1}$ and $p_{i+1}$ (or just one if at end of chain) \;
	%     }
	%     \If{$\textit{cmd} = (\cmdEject, \textup{post-payment transaction of any channel in the chain})$} {
	%         $\stage \gets \stageTerminated$ \; 
	%         return post-payment settlements for channels with $p_{i-1}$ and $p_{i+1}$ (or just one if at end of chain) \;
	%     }
	% }
	
	\KwOn({\cmdEject}) {
		\label{alg:eject}
		
		%\assertx{
		%	\textit{No \popt was placed on the blockchain}
		%}
		
		\assign{s}{\channel{stage}{p_i}{p_{i+1}}} \;
		\assign{\channel{stage}{p_i}{p_{i+1}}}{\stageTerminated} \;
		
		\If{$\mathit{s} = \cmdLockAlg \lorx \mathit{s} = \cmdSignAlg \lorx \mathit{s} = \cmdUpdateAlg \lorx \mathit{s} = \cmdReleaseAlg$} {
		\genblocktx{\Return \channel{current\_tx}{p_{i-1}}{p_i} and \channel{current\_tx}{p_{i}}{p_{i+1}} \; \label{alg:eject:ind}
		}}
		
		\genblocktx{\Return \signedChainSettleTx \label{alg:eject:all}
	}}\BlankLine 
	
	\KwOn({$\cmdEject(\mathit{popt})$}) {
		\label{alg:eject_popt}
		
		%\assertx{
		%	\textit{$\mathit{popt}$ was placed on the blockchain}
		%}
		
		\assign{s}{\channel{stage}{p_i}{p_{i+1}}} \;
		\assign{\channel{stage}{p_i}{p_{i+1}}}{\stageTerminated} \;
		
		\If{$\mathit{popt} = \cmdLockAlg \lorx \mathit{popt} = \cmdSignAlg$} {
		\genblocktx{\Return \channel{pre\_pay\_tx}{p_{i-1}}{p_i} and \channel{pre\_pay\_tx}{p_{i}}{p_{i+1}}\; \label{alg:eject_popt:pre}    
		}}
		
		\ElseIf{$\mathit{popt} = \cmdUpdateAlg \lorx \linebreak \mathit{popt} = \cmdReleaseAlg$} {
		\genblocktx{\Return \channel{post\_pay\_tx}{p_{i-1}}{p_i} and \channel{post\_pay\_tx}{p_{i}}{p_{i+1}} \label{alg:eject_popt:post}
		}}
	 }
	 \end{multicols}
	\vspace*{1em}
\end{algorithm*}


==> algo4.tex <==
\newcommand{\msgNewChannelAckAlg}{\algCmd{\msgNewChannelAck}}		
\newcommand{\msgApproveMyDepositAlg}{\algCmd{\msgApproveMyDeposit}}		
\newcommand{\msgApprovedDepositAlg}{\algCmd{\msgApprovedDeposit}}	
\newcommand{\msgAssociatedDepositAlg}{\algCmd{\msgAssociatedDeposit}}
\newcommand{\msgPaidAlg}{\algCmd{\msgPaid}}
\newcommand{\msgDissociatedDepositAlg}{\algCmd{\msgDissociatedDeposit}}
\newcommand{\msgDissociatedDepositAckAlg}{\algCmd{\msgDissociatedDepositAck}}
		\begin{algorithm*}[ht]\scriptsize
			\caption{\sys payment channel protocol
                          {\footnotesize{}(For brevity, we constrain deposits
                            to be paid into $1$-out-of-$1$ multisignature
                            addresses; \cref{sec:ft:bft} outlines the protocol
                            for general $m$-out-of-$n$ deposits. We omit
                            freshness protection of messages.)}
                       } 
			\label{alg:teechainChannelA}
			\SetAlgoNoEnd
			\DontPrintSemicolon 
			\SetNoFillComment
			\SetAlgoNoEnd
			\SetInd{0.4em}{0.4em}
%			\vspace*{-2em}
			\begin{multicols}{3}
%				\commentx{} \;
				$(\myPubKey, \myPrivKey) \gets$ generate public, private keys {\label{alg:line:pubpriv}} \;
				%\BlankLine
				
				$\forall \pubKey: \networkChannelAESKey(\pubKey) = \bot$
				\commentx{AES keys for network channels}
				%\BlankLine
				
				$\forall \channelID: \channelPubKey(\textit{\channelID}) = \bot$ \commentx{Remote pub keys} \;
				{\label{alg:line:aeskey}}
				$\forall \channelID: \channelIsReady(\channelID) = False$ \commentx{Pay chans closed}\;
				%\BlankLine
				%\BlankLine
				
				$\forall \channelID: \channelMyDeposit(\channelID) = \bot$ \commentx{My deposits in pay chan}\; 
				$\forall \channelID: \channelTheirDeposit(\channelID) = \bot$ \commentx{Remote deps in pay chan}\; 
				$\forall \channelID: \channelMyBalance(\channelID) = \bot$ \commentx{My bal in pay chan}\;
				$\forall \channelID: \channelTheirBalance(\channelID) = \bot$ \commentx{Remote bal in pay chan}\; 
				$\forall \channelID: \channelMyAddress(\channelID) = \bot$  \commentx{My Bitcoin addresses}\;
				$\forall \channelID: \channelTheirAddress(\channelID) = \bot$ \commentx{Remote Bitcoin addresses}\;
				$\forall \textit{tx}: \deposits(\textit{tx}) = \bot$
				\commentx{All tx output deposits}\;
				$\forall \textit{tx}: \freeDeposits(\textit{tx}) = \bot$ \commentx{Unassociated deposits}\;
				$\forall \pubKey: \approvedDeposits(\pubKey) = \bot$ 
				\commentx{Remote approved deps}\;
				$\forall \btcAdd: \bitcoinPrivateKeys(\btcAdd) = \bot$ 
				\commentx{Btc private keys}\;				
				
				\BlankLine 
				
				\KwOn({$\cmdNewNetworkChannel(\remotePubKey)$}) {\label{alg:newnetworkchannel} 
					assert $\networkChannelAESKey(\remotePubKey) = \bot$ \;
					$\networkChannelAESKey(\remotePubKey) \gets$ \textit{remote attestation and authenticated Diffie-Hellman using \remotePubKey} \label{alg:dh} \; 
				} 
				%\BlankLine

				\BlankLine 				
				
				\KwOn({$\cmdNewPaymentChannel(\channelID, \remotePubKey, \remoteBtcAdd, \myBtcAdd)$}) {\label{alg:line:cmdnewchannel} 
					assert $\channelPubKey(\channelID) = \bot$ \;
					$\channelPubKey(\channelID) \gets \remotePubKey$ \;
					$\channelMyAddress(\channelID) \gets \myBtcAdd$ \; 
					$\channelTheirAddress(\channelID) \gets \remoteBtcAdd$ \; 
					$\channelMyBalance(\channelID) \gets 0$ \; 
					$\channelTheirBalance(\channelID) \gets 0$ \; 
					$\channelIsReady(\channelID) \gets \vFalse$ \; 
					return $(\msgNewChannelAckAlg, \channelID, \myBtcAdd, \remoteBtcAdd)$ signed by $\textit{\myPrivKey}$ \label{alg:line:newchannelack} \;
					%and encrypted under $\networkChannelAESKey(\textit{theirPubKey})$
				} 
				%\BlankLine 
				\BlankLine 
				
				\KwOn({\cmdReceive[] $(\msgNewChannelAckAlg, \channelID, \remoteBtcAdd, \myBtcAdd)$ signed by \privKey for \channelPubKey(\channelID)}) {\label{alg:line:cmdnewchannel:ack}
					assert $\channelIsReady(\channelID) = \vFalse$ \; 
					assert $\channelMyAddress(\channelID) = \myBtcAdd$ \; 
					assert $\channelTheirAddress(\channelID) = \remoteBtcAdd$ \; 
					$\channelIsReady(\channelID) \gets \vTrue$ \; 
				} 
				%\BlankLine 
				\BlankLine 
				
				\KwOn({$\cmdGetAddr()$}){\label{alg:getaddr}
					$\textit{(\btcAdd,\btcPrivKey)} \gets$ new Bitcoin address and private key \;
					\encalg{$\bitcoinPrivateKeys(\btcAdd) \gets \btcPrivKey$}\label{alg:btcnewkey} \;
					return \btcAdd
				} 
				%\BlankLine 
				\BlankLine 
				
				\KwOn({$\cmdNewDeposit(\textit{txo},\btcAdd)$}){\label{alg:newdeposit}
					assert $\bitcoinPrivateKeys(\btcAdd)$ exists \; 
					assert $\textit{txo} \not\in \deposits$ \commentx{can't add same dep twice}\;
					assert $\textit{txo.btcAddress = \btcAdd}$ \commentx{verify txo}  \;
					$\deposits \gets \deposits \cup \{ \textit{txo} \}$ \; 
					$\freeDeposits \gets \freeDeposits \cup \{ \textit{txo} \}$ \;
				} 
				%\BlankLine 
				\BlankLine 
				
				\KwOn({$\cmdRemoveDeposit(\textit{txo}, \btcAdd)$}){\label{alg:removedeposit}
					assert $\textit{txo} \in \freeDeposits$ \commentx{verify deposit is free}\;
					assert $\bitcoinPrivateKeys(\textit{txo.bitcoinAddress})$ exists \;
					\genblocktx{$\textit{tx} \gets$ generate tx spending \textit{txo} into \btcAdd using $\bitcoinPrivateKeys(\textit{txo.btcAddress})$} \label{alg:returndep}\; 
					$\freeDeposits \gets \freeDeposits \setminus \{ \textit{txo} \}$ \; 
					return \textit{tx} \; 
				} 
				%\BlankLine
				\BlankLine 
				
				\KwOn({$\cmdApproveMyDeposit(\remotePubKey, \textit{txo})$}) {\label{alg:approvemydeposit}
					assert $\networkChannelAESKey(\remotePubKey)$ exists \;
					assert $\textit{txo} \in \freeDeposits$ \;
					assert $\textit{txo} \not\in \approvedDeposits(\remotePubKey)$ \; 
					return $(\msgApproveMyDepositAlg, \myPubKey, \textit{txo})$ signed by \myPrivKey.
				}
				\BlankLine 
				
				\KwOn({\cmdReceive[] $(\msgApproveMyDepositAlg,\remotePubKey, \textit{txo})$ signed by \privKey for \remotePubKey}) {\label{alg:line:approvetheirdeposit}
					assert $\networkChannelAESKey(\remotePubKey)$ exists \;
					assert $\textit{txo} \not\in \approvedDeposits(\remotePubKey)$ \;
					\genblocktx{Verify that \textit{txo} is in the blockchain} \;
					$\approvedDeposits{(\remotePubKey)} \gets \approvedDeposits{(\remotePubKey)} \cup \{ \textit{txo} \}$ \;
					return $(\msgApprovedDepositAlg, \myPubKey, \textit{txo})$ signed using $\textit{\myPrivKey} \label{alg:depositapprov}$
				} 
				
				\BlankLine 
				
				\KwOn({$\cmdReceive(\msgApprovedDepositAlg, \remotePubKey, \textit{txo}))$ signed by \privKey for \remotePubKey}) {\label{alg:receive:approved}
					assert $\networkChannelAESKey(\remotePubKey)$ exists \;
					assert $\textit{txo} \in \freeDeposits$ \;
					assert $\textit{txo} \not\in \approvedDeposits(\remotePubKey)$ \;
					$\approvedDeposits{(\remotePubKey)} \gets \approvedDeposits{(\remotePubKey}) \cup \{ \textit{txo} \}$ \;
				} 
				\BlankLine 
				
				
				\KwOn({$\cmdAssociateMyDeposit(\channelID, \textit{txo})$}) {\label{alg:assocmydeposit}
					assert $\channelIsReady(\channelID) = \vTrue$\; 
					assert $\textit{txo} \in \approvedDeposits(\channelPubKey(\channelID))$ \;
					assert $\textit{txo} \in \freeDeposits$ \;
					$\freeDeposits \gets \freeDeposits \setminus \{ \textit{txo} \}$ \;
					$\channelMyDeposit(\channelID) \gets \channelMyDeposit(\channelID) \cup \{ \textit{txo} \}$ \;
					$\channelMyBalance(\channelID) \gets \channelMyBalance(\channelID) + \textit{txo.amount}$ \label{alg:assocbalreq} \;
					$\remotePubKey \gets$ $\channelPubKey(\channelID)$ \;
					\encalg{$\encBtcPrivKey \gets$ $\bitcoinPrivateKeys(\textit{txo.btcAddress})$ encrypted under $\networkChannelAESKey(\remotePubKey)$} \label{alg:btcsharekey} \;
					return $(\msgAssociatedDepositAlg, id, \textit{txo}, \encBtcPrivKey)$ signed using $\myPrivKey$ \label{alg:assocreq} 
					%and encrypted under $\networkChannelAESKey(\textit{theirPubKey})$    
				} 
				\BlankLine 
				
				
				\KwOn({$\cmdReceive(\msgAssociatedDepositAlg, \channelID, \textit{txo}, \encBtcPrivKey)$ signed by \privKey for \channelPubKey(\channelID)})
				{\label{alg:assoctheirdeposit}
					assert $\channelIsReady(\channelID) = \vTrue$ \;
					assert $\textit{txo} \in \approvedDeposits(\channelPubKey(\channelID))$ \;
					$\channelTheirDeposit(\channelID) \gets \channelTheirDeposit(\channelID) \cup \{ \textit{txo} \}$ \;
					$\channelTheirBalance(\channelID) \gets \channelTheirBalance(\channelID) + \textit{txo.amount}$ \;
					$\remotePubKey \gets$ $ \label{alg:assocbal} \;
					\channelPubKey(\channelID)$ \;
					\encalg{$\btcPrivKey \gets$ \encBtcPrivKey decrypted under $\networkChannelAESKey(\remotePubKey)$} \;
					$\bitcoinPrivateKeys(\textit{txo.btcAddress}) \gets \btcPrivKey $
				} 
				\BlankLine 
				
				\KwOn({$\cmdPay(\channelID, \textit{amount})$}) {\label{alg:fix:pay}
					%     \If({\hfill (We read \channelMyDeposit as the amount)}) {$\channelMyBalance(\textit{channelID}) - \textit{amount} \le \channelMyDeposit(\textit{channelID})$} {
					assert $\channelMyBalance(\channelID) \geq \textit{amount}$ \;
					$\channelMyBalance(\channelID) \gets \channelMyBalance(\channelID) - \textit{amount}$ \; 
					$\channelTheirBalance(\channelID) \gets \channelTheirBalance(\channelID) + \textit{amount}$ \; 
					return $(\msgPaidAlg, \channelID, \textit{amount})$ signed using $\myPrivKey$ \label{alg:pay:not}  \;
					%     }
				} 
				\BlankLine 
				
				\KwOn({$\cmdReceive(\msgPaidAlg, \channelID, \textit{amount})$ signed by \privKey for \linebreak \channelPubKey(\channelID)}) {\label{alg:receive:pay}
					$\channelMyBalance(\channelID) \gets \channelMyBalance(\channelID) + \textit{amount}$ \;
					$\channelTheirBalance(\channelID) \gets \channelTheirBalance(\channelID) - \textit{amount}$ \; 
				}
				\BlankLine 
				
				\KwOn({$\cmdDissociateMyDeposit(\channelID, \textit{txo})$}) {\label{alg:dissociate} 
					assert $\textit{txo} \in \channelMyDeposit(\channelID)$ \; 
					assert $\channelMyBalance(\channelID) \geq \textit{txo.amount} $ \;
					return $(\msgDissociatedDepositAlg, \channelID, \textit{txo})$ signed \linebreak using $\myPrivKey$
				} 
				\BlankLine 
				
				\KwOn({\cmdReceive$(\msgDissociatedDepositAlg, \channelID, \textit{txo})$ \linebreak signed by \privKey for \channelPubKey(\channelID)}) {\label{alg:dissociate:msg}
					assert $\textit{txo} \in \channelTheirDeposit(\channelID)$ \; 
					assert $\channelTheirBalance(\channelID) \geq \textit{txo.amount}$ \;
					$\channelTheirDeposit(\channelID) \gets \channelTheirDeposit(\channelID) \setminus \{ \textit{txo} \}$ \;
					$\channelTheirBalance(\channelID) \gets \channelTheirBalance(\channelID) - \textit{txo}$ \; 
					return $(\msgDissociatedDepositAckAlg, \channelID, \textit{txo})$ \linebreak signed using $\myPrivKey$ \label{alg:dissociate:ackreq} \;
				} 
				\BlankLine 
				
				\KwOn({\cmdReceive[\scriptsize] $(\msgDissociatedDepositAckAlg, \channelID, \textit{txo})$ \linebreak signed by \privKey for \channelPubKey(\channelID)}) {\label{alg:dissociate:ack}
					$\channelMyDeposit(\textit{pubKey}) \gets \channelMyDeposit(\textit{pubKey}) \setminus \{ \textit{txo} \}$ \;
					$\channelMyBalance(\channelID) \gets \channelMyBalance(\channelID) - \textit{txo}$ \;
					$\freeDeposits \gets \freeDeposits \cup \{ \textit{txo} \}$ \;
					\encalg{$\bitcoinPrivateKeys(\textit{txo.btcAddress}) \gets \bot$} \label{alg:btcremkey}
				} 
				\BlankLine 
				
				\KwOn({$\cmdSettle(\channelID)$}) {\label{alg:settle}
					\If{$\channelMyBalance(\channelID) = \sum_{1}^{n}{(\channelMyDeposit(\channelID)\textit{.amount})} \land \linebreak \channelTheirBalance(\channelID) = \sum_{1}^{n'}{(\channelTheirDeposit(\channelID)\textit{.amount)}})$} {
					    $\forall \textit{tx}$ in $ \channelMyDeposit(\channelID): \textit{dissociateDeposit}(\textit{tx})$ \label{alg:settle:off}\;
					    Notify remote to dissociate all deposits. \;
					}
					
					\If{$\channelMyDeposit(\channelID) = \bot \land \channelTheirDeposit(\channelID) = \bot$} {
						\commentx{Remote dissociated deps. \\Terminate off-chain.} \;
						$\forall \textit{i}: \channelI(\channelID)\gets \bot$ \commentx{Reset all channel state}\;
					} \Else {
						\textit{allDepAddrs} $\gets \forall \textit{tx}$ in $(\channelMyDeposit(\channelID) \cup \channelTheirDeposit(\channelID)): \textit{return tx.btcAddress}$ \;
					 	\genblocktx{$\textit{tx} \gets$ generate signed \textit{txo} spending:}\label{alg:settle:gen} \; \channelMyBalance(\channelID) into \channelMyAddress(\channelID) \& \;
					\channelTheirBalance(\channelID) into \channelTheirAddress(\channelID) using: \;
					$\bitcoinPrivateKeys{(\textit{allDepAddrs})}$ \; 		
					$\forall \textit{i}: \channelI(\channelID)\gets \bot$
					\commentx{Reset all channel state}\;
					Notify remote that I terminated. \;
				    return \textit{tx} \; \label{alg:on:settle}
					}
				} 
				\BlankLine 
			\end{multicols}
			\vspace{0.5em}	
		\end{algorithm*} % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
